On the Approximability of Related Machine Scheduling under Arbitrary Precedence

Distributed computing systems often need to consider the scheduling problem involving a collection of highly dependent data-processing tasks that must work in concert to achieve mission-critical objectives. This paper considers the unrelated machine scheduling problem for minimizing weighted sum completion time under arbitrary precedence constraints and on heterogeneous machines with different processing speeds. The problem is known to be strongly NP-hard even in the single machine setting. By making use of Queyranne's constraint set and constructing a novel Linear Programming relaxation for the scheduling problem under arbitrary precedence constraints, our results in this paper advance the state of the art. We develop a $2(1+(m-1)/D)$-approximation algorithm (and $2(1+(m-1)/D)+1$-approximation) for the scheduling problem with zero release time (and arbitrary release time), where $m$ is the number of servers and $D$ is the task-skewness product. The algorithm can be efficiently computed in polynomial time using the Ellipsoid method and achieves nearly optimal performance in practice as $D>O(m)$ when the number of tasks per job to schedule is sufficiently larger than the number of machines available. Our implementation and evaluation using a heterogeneous testbed and real-world benchmarks confirms significant improvement in weighted sum completion time for dependent computing tasks.

==> 1_background.tex <==
\section{Background and motivation} \label{sec:background}





==> 3_approximation_algorithm.tex <==
\section{approximation algorithm} \label{sec:approximation_algorithm}


%We consider an offline jobs scheduling problem with release time. Consider given positive weight parameters $w_j$, $j=1,2,...,N$. Our objective is to minimize the total weighted completion time of all jobs, \ie $\min\sum w_j C_j$. We first present a core linear program (LP-MapReduce) that is used in the algorithm to order jobs. Then, we describe our algorithm, which can order jobs and give scheduling scheme for each job.

In this section, we develop an algorithm to solve the weighted completion time minimization problem on heterogeneous machines  and under precedence constraints. The algorithm is based on first solving a linear optimization, referred to as the LP-MapReduce problem. The solution is then used to obtain a feasible schedule executing map and reduce tasks on the machines.


\subsection{LP-MapReduce}
%In this subsection, we will formulate a linear program LP-MapReduce, whose solution will be used to give the approximation algorithm.  
We formulate the LP-MapReduce as follows: 


\begin{equation}
	\min \sum_{j\in\mathcal{N}}w_jC_{j} 
\end{equation}

subject to:
\begin{eqnarray}
	&&\sum_{j\in {\mathcal{S}}}p_{j} C_j \geq \frac{\left(\sum_{j\in {\mathcal{S}}}p_j\right)^2}{2\mu}+\sum_{j\in {\mathcal{S}}}\frac{\left(p_j\right)^2}{2\mu_j}   \forall {\mathcal{S}} \subseteq \mathcal{N} \label{const1}\\
	%$\sum_{j\in S}p_{j}^\diamond C_j^\diamond\geq\frac{1}{2}\Big{[}\frac{(\sum_{j\in S}p_j^\diamond)^2}{\mu}+\sum_{j\in S}\frac{(p_j^\diamond)^2}{\mu_j}\Big{]}$~~$\forall S\subset [N]$
	&&C_j^M \geq p_{j,t}^M/v_1+r_{j}\ \  \forall j\in\mathcal{N}, t\in T_j^M  \label{const2}\\
	&&C_j \geq p_{j,t}^R/v_1+C_{j}^M\  \  \forall j\in\mathcal{N}, t\in T_j^R \label{const3}\\
	&&C_j^M \geq p_{j}^M/\mu_j+r_{j}\  \   \forall j\in\mathcal{N} \label{const4}\\
	&&C_j \geq p_{j}^R/\mu_j+C_{j}^M\  \   \forall j\in\mathcal{N} \label{const5}
\end{eqnarray}



We note that constraint \eqref{const1} is based on the Queyranne's constraint set \cite{queyranne1993structure}, which has been used to give 2-approximation for concurrent open shop scheduling \cite{leung2007scheduling,mastrolilli2010minimizing} without precedence constraints. The extension to machines with different processing speeds is due to \cite{murray2016scheduling}, which formulated different versions of the polyhedral constraints based on Queyranne's constraint set. Our constraint \eqref{const1} is similar to that in \cite{murray2016scheduling}, but now applied to reduce job completion times, because all map tasks must be completed before reduce tasks under precedence constraints, and thus, $C_j$ is also the completion time of the entire job $j$. While \eqref{const1} does not explicitly force map tasks to finish before reduce jobs, it states that the completion of a job implies finishing all its map and reduce tasks.

%since all the tasks of the map and of the reduce must be completed for the completion of the job and thus the processing time of the job is the sum of all the tasks.  Using the result in \cite{murray2016scheduling}, we see that every feasible solution to the proposed problem must satisfy the constraint  \eqref{const1}. We further note that \eqref{const1} do not explicitly constrain that the map jobs should be complete before the reduce jobs. This constraint depicts that the completion of a job implies completion of all the map and reduce tasks.


%use the same constraint as in \cite{murray2016scheduling} for the set of tasks with a key difference. The difference is that we have $2N$ sub-jobs, $N$ map sub-jobs and $N$ reduce sub-jobs. In the choice of all subset of jobs, we choose a map sub-job and reduce sub-job of the same job together and use the constraint. Ideally, the set ${\mathcal{S}}$ of map sub-jobs can be chosen different from the set ${\mathcal{S}}$ for the reduce sub-jobs. Choosing the two as the same helps reduce complexity, while the approximation guarantee can still be shown as will be shown in Section \ref{sec:proof}. Using the result in \cite{murray2016scheduling}, we see that every feasible solution to the proposed problem must satisfy the constraint  \eqref{const1}. 


Constraint \eqref{const2} means that the completion time of all map tasks is at least the release time (\ie the earliest time job $j$ can begin processing) plus the required processing time of any map task $t$ on the fastest machine (\ie the minimum required processing time of any map task). Similarly, constraint \eqref{const3} requires the completion time of all reduce tasks to be at least the completion time of all map tasks plus the time needed to finish any reduce tasks on the fastest machine. This is due to the precedence constraint, forcing reduce tasks to start after all map tasks are finished. Finally, constraint \eqref{const4} implies that the time required to process all map tasks (\ie from $r_j$ to $C_J^M$) is at least the total data size $P_j^M$ of all the map tasks divided by the maximum possible processing speed $\mu_j$ of job $j$. Similarly, \eqref{const5} means that the reduce task completion time $C_j$ must be at least the completion time of all map tasks plus the minimum processing time of all reduce tasks, given by the total data size of all reduce tasks divided by the maximum possible processing speed of job $j$. We note that the constraints \eqref{const2}-\eqref{const5} do not account for multiple jobs this providing loose bounds. Furthermore, we also note that the constraints \eqref{const2}-\eqref{const5} can be made concise by reducing to a single combined constraint:
\begin{eqnarray}
C_j &\geq& \max(p_{j}^R/\mu_j,\max_{t\in T_j^R}p_{j,t}^R/v_1) +r_{j}\nonumber\\
&&+\max(p_{j}^M/\mu_j,\max_{t\in T_j^M}p_{j,t}^M/v_1)\ \  \forall j\in\mathcal{N}.   \label{const6}
\end{eqnarray}



%Constraint \eqref{const3} is similar to \eqref{const2}, except for the reduce sub-job rather than map sub-job and the release time for the reduce job is the completion time of the map sub-job. Constraint \eqref{const4}  states that the completion time of a map sub-job is at least the release time plus the ratio of the processing times of all the tasks of the map sub-job and the sum of speeds of the fastest $q_j^M$ machines. This is because if all the tasks are combined together and the resources of the best machines are pulled together, the time taken will be lower than the actual time taken to process the jobs. Constraint \eqref{const5}  is similar to \eqref{const4}, except for the reduce sub-job rather than map sub-job and the release time for the reduce job is the completion time of the map sub-job. The constraints \eqref{const2}-\eqref{const5} do not account for multiple jobs, are valid when there is only a single job $j$ that need to be processed. We also note that the constraints \eqref{const2}-\eqref{const5} can be made concise and reduced to a total of $N$ constraints given as



Because constraints \eqref{const1} and \eqref{const6} are necessary for any feasible solution of the weighted completion time optimization, any optimal solution of the LP-MapReduce provides a lower bound for the weighted completion time optimization. This lower bound may not be tight, and the optimal solution may not be feasible in the original optimization, since LP-MapReduce does not take into account all sufficient constraints. Nevertheless, we show that a feasible schedule for executing map and reduce tasks on different machines can be obtained from the optimal solution of the LP-MapReduce. 

%as compared to the optimal solution. Further, since all the possible constraints are not enumerated, the solution of LP-MapReduce is not the optimal solution for the original problem. In addition, the solution to the problem does not give a schedule for assignment of different tasks to different servers. Thus, we will give a scheduling algorithm based on the solution to the optimization problem in LP-MapReduce.

%We also note that although the precedence constraints are only partially considered in \eqref{const1}-\eqref{const5} (since these constraints are necessary but not sufficient), our proposed scheduling algorithm relying on the optimal solution of LP-MapReduce can still yield a solution to the weighted completion time optimization with a guaranteed approximation ratio.

We note that in the proof of the approximation ratio, we only use the constraints \eqref{const1} and $C_j \geq p_{j}/\mu_j+r_{j}$ (which follows from \eqref{const6}). These constraints do not consider the precedence constraints and only account for all the map-reduce tasks being completed from the servers. Thus, even though the LP formulation with these two constraints do not account for the precedence constraints, we note that the proposed algorithm will be shown to have approximation guarantees in the case when the precedence constraints are present. 

%in the presence of the precedence constraints.

%We note that the problem formulation of LP-MapReduce which minimizes $\sum_{j\in[N]}w_jC_{j}$ such that \eqref{const1} and \eqref{const6} does not account for the two-stage problem of map-reduce since these constraints do not explicitly constrain that the map jobs should be complete before the reduce jobs. These constraints depict that the completion of a job implies completion of all the map and reduce tasks.


\subsection{Complexity of Solving LP-MapReduce}

At a first look, even though LP-MapReduce is a linear program, the constraint \eqref{const1} takes every possible subset of $\mathcal{N}$ and thus contains $O(2^N)$ different constraints, one for each $\mathcal{S}\subseteq \mathcal{N}$. We show that utilizing a special structure of these linear constraints, the LP-MapReduce problem can actually be solved in polynomial time. To this end, we make use of the Ellipsoid method \cite{grotschel1981ellipsoid}, which needs a separation oracle to determine the  violated constraint. In order to find such a separation oracle, we will first determine the most violated constraint in \eqref{const1} since there are only $N$ other constraints in \eqref{const6}.   Let the violation $V(\mathcal{S})$ for a set ${\mathcal{S}} \subseteq \mathcal{N}$ be defined as follows. 
\begin{equation}	
V(\mathcal{S}) =-\sum_{j\in {\mathcal{S}}}p_{j} C_j +\frac{1}{2\mu} \left(\sum_{j\in {\mathcal{S}}}p_j\right)^2 +\frac{1}{2}\sum_{j\in {\mathcal{S}}}\frac{\left(p_j\right)^2}{\mu_j}
	\end{equation}

Let $\{C_j\}$ for all $j$ be a potentially feasible solution to LP-MapReduce. Let $\sigma$ denote the ordering when jobs
are sorted in an increasing order of $C_j  - p_j/(2μ_j)$. Find the most violated constraint in \eqref{const1}  by searching over $V(\mathcal{S})$ for $\mathcal{S}$ of the form $\{\sigma(1), \cdots, \sigma(j)\}$, $j\in \{1, \cdots, N\}$. If any of maximal $V(\mathcal{S}) > 0$, then return $\mathcal{S}$ as a violated constraint for \eqref{const1}. Otherwise,
check the remaining $N$ constraints \eqref{const6} directly in linear time.

Oracle-LP  finds the subset of jobs that maximizes the ``violation". That is, Oracle-LP finds $\mathcal{S}^*$ such that $V(\mathcal{S}^*) = \max_{\mathcal{S}\subseteq \mathcal{N}}V(\mathcal{S})$. We prove the correctness
of Oracle-LP by establishing a necessary and sufficient condition for a job $j$ to be in $\mathcal{S}^*$.

\begin{lemma}\label{lem:oracle}
	Let ${\mathbb P}(\mathcal{A}) \triangleq \sum_{j\in {\mathcal{A}}} p_j$. Then, we have $x\in \mathcal{S}^* \iff C_x - p_x/2\mu \le {\mathbb P}(\mathcal{S}^*)/\mu $
\end{lemma}
\begin{proof}
	The proof follows on the same lines as in \cite{murray2016scheduling} and is thus omitted.
\end{proof}


Given Lemma \ref{lem:oracle}, it is easy to verify that sorting jobs in increasing order of $C_x-p_x/(2\mu_x)$ to define a permutation $\sigma$ guarantees that $\mathcal{S}^*$ is of the form $\{\sigma(1), \cdots, \sigma(j)\}$ for
some $j\in \mathcal{N}$. This implies that  Oracle-LP finds $\mathcal{S}^*$ in $O(N \log(N))$ time.  Since the remaining constraint \eqref{const6} can be verified in linear time,  Oracle-LP runs in $O(N\log(N))$ time. Thus, the LP-MapReduce problem with Ellipsoid method \cite{grotschel1981ellipsoid} using the above separation oracle is solvable in polynomial time. 

% map tasks of a job can start to run only after the job is released, and the amount of processing time should be larger than the processing time of any task in the fastest machine. Constraints (\ref{const3}) state that reduce tasks of a job can start to run only after all map tasks of the job finish, and the amount of processing time should be larger than the processing time of any task in the fastest machine. Constraints (\ref{const4}) state that map tasks of a job can start to run only after the job is released, and the amount of processing time should be larger than the processing time of all map tasks in the fastest $\mu_j^M$ machines. Constraints (\ref{const5}) state that reduce tasks of a job can start to run only after all map tasks of the job finish, and the amount of processing time should be larger than the processing time of all map tasks in the fastest $\mu_j^R$ machines. We note that these constraints are necessary for the overall problem.

\subsection{Proposed Algorithm}
Let $\{C_j\}$ $\forall j$ be the optimal completion times found by the LP-MapReduce algorithm. Our algorithm to identify a feasible schedule for the weighted completion time optimization consists of the following steps. First, we sort the $N$ jobs, with respect to $C_j - p_j/2\mu_j$, in an ascending order. The $N$ sorted jobs are labeled $\sigma(1)$, $\cdots$, $\sigma(N)$ where $\sigma$ is the corresponding permutation of the $N$ jobs. Next, we schedule map and reduce tasks one-by-one, beginning with map tasks from the one with highest processing data size to the lowest (\ie for $t=1,2,\ldots, |T_{\sigma(j)}^M|$), and then scheduling reduce tasks in the same order. When scheduling each (map or reduce) task $t$, we assign it to a machine that produces the earliest completion time, with respect to all tasks already assigned to the machine, the task $t$'s release time, and the required processing speed of task $t$ on the machine. Finally, once all (map and reduce) tasks are assigned, the order of task executions on each machine is determined. We then insert idle time on all machines as necessary, if any job's reduce tasks have an earlier starting time than the completion of all its map tasks, and if any jobs begin processing ahead of its release time. This procedure ensures the precedence constraints between map and reduce tasks, as well as the feasibility of job starting times. The pseudocode of our proposed Dependent Map-Reduce Scheduling (DMRS) algorithm is shown in Algorithm~\ref{alg1}.


%The jobs are scheduled in order with all the map or reduce tasks scheduled. The order of tasks is from the first (highest processing size) to the last task (lowest processing size) with the map tasks before the reduce tasks. When placing a particular task, assign it whichever machine and start time results in the task being completed as early as possible (without moving any tasks which have already been placed). Insert idle time (on all $m$ machines) as necessary if this procedure would otherwise start a job before its release time (or finishing of all map  tasks of the job before reduce tasks start). The pseudocode is shown in Algorithm~\ref{alg1}.
\vspace{-.1in}
\begin{algorithm}
	\caption{{\sc Proposed DMRS Algorithm}}
	\label{alg1}
	\begin{algorithmic}[1]
		%\STATE{Inputs:}
		%\STATE{Outputs:}
		\STATE{Find optimal $C_j$ $\forall j$ by solving LP-MapReduce}
		\STATE{Sort jobs to find $\sigma(1),\ldots,\sigma(N)$ in ascending order with respect to $C_{\sigma(j)} - p_{\sigma(j)}/2\mu_{\sigma(j)}$}
		\STATE{Initialize $t_l=0$ for all machines $l=1,\ldots,m$}
		\STATE{{\bf for} jobs $j=1$ to $N$}
		\STATE{ \ \ \ {\bf for} map tasks $t=1$ to $|T_{\sigma(j)}^M|$}  
		\STATE{ \ \ \ \ \ \ $l^*={\rm arg}\min_l \left\{\max(t_{l},r_{\sigma(j)}) + p_{\sigma(j),t}^M/v_l\right\}$ }
		 \STATE{ \ \ \ \ \ \ Assign map task $t$ to machine $l^*$}
		 \STATE{ \ \ \ \ \ \ Update $t_{l^*} \leftarrow \max(t_{l^*},r_{\sigma(j)}) + p_{\sigma(j),t}^M/v_{l^*}$ }
		\STATE{\ \ \ {\bf end for} }
		\STATE{\ \ \ Find completion time $T_{\sigma(j)}^M$ of job $\sigma(j)$'s map tasks}
		\STATE{ \ \ \ {\bf for} reduce tasks $t=1$ to $|T_{\sigma(j)}^R|$}  
		\STATE{ \ \ \ \ \ \ Let $\tau_l = \max(t_l,T_{\sigma(j)}^M, r_{\sigma(j)}), \ \forall l$}
		\STATE{ \ \ \ \ \ \ $l^*={\rm arg}\min_l \left\{\tau_l+ p_{\sigma(j),t}^R/v_l\right\}$}
		\STATE{ \ \ \ \ \ \ Assign reduce task $t$ to machine $l^*$}
		 \STATE{ \ \ \ \ \ \ Update $t_{l^*} \leftarrow \tau_{l^*} + p_{\sigma(j),t}^R/v_{l^*}$ }
		\STATE{\ \ \ {\bf end for}}
		\STATE{{\bf end for}}
	\end{algorithmic}
\end{algorithm}



==> abstract.tex <==
\begin{abstract}
Distributed computing systems often need to consider the scheduling problem involving a collection of highly dependent data-processing tasks that must work in concert to achieve mission-critical objectives. This paper considers the unrelated machine scheduling problem for minimizing weighted sum completion time under arbitrary precedence constraints and on heterogeneous machines with different processing speeds. The problem is known to be strongly NP-hard even in the single machine setting. By making use of Queyranne's constraint set and constructing a novel Linear Programming relaxation for the scheduling problem under arbitrary precedence constraints, our results in this paper advance the state of the art. We develop a $2(1+(m-1)/D)$-approximation algorithm (and $2(1+(m-1)/D)+1$-approximation) for the scheduling problem with zero release time (and arbitrary release time), where $m$ is the number of servers and $D$ is the task-skewness product. The algorithm can be efficiently computed in polynomial time using the Ellipsoid method and achieves nearly optimal performance in practice as $D>O(m)$ when the number of tasks per job to schedule is sufficiently larger than the number of machines available. Our implementation and evaluation using Hadoop confirms significant improvement in weighted sum completion time for dependent computing tasks.
%MapReduce is the most popular big-data computation framework, motivating many research topics. A MapReduce job consists of two successive phases, \ie map phase and reduce phase. Each phase can be divided into multiple tasks. A reduce task can only start when  all the map tasks finish processing. A job is successfully completed when all its map and reduce tasks are complete. The task of optimally scheduling the different tasks on different servers to minimize the weighted completion time is an open problem, and is the focus of this paper. In this paper, we give an approximation ratio with a competitive ratio $2(1+(m-1)/D)+1$, where $m$ is the number of servers and $D\ge 1$ is the task-skewness product. We implement the proposed algorithm on Hadoop framework, and compare with three baseline schedulers. Results show that our DMRS algorithm can outperform baseline schedulers by up to $82\%$.
\end{abstract}


==> approx_results.tex <==
\section{Proof of DMRS Approximation Ratio}\label{sec:proof}

We analyze the approximation ratio of DMRS algorithm. Let $\widehat{C}_j$ be the completion time of job $j$ from the proposed DMRS algorithm. 

 %(Slight adaptations can be used for analyzing Algorithm 1). 

\begin{lemma}\label{lemused}
Suppose $N$ jobs are scheduled using DMRS. The completion time of job $\sigma(j)$, for all $j= 1, \cdots, N$, satisfy
\begin{eqnarray}
\widehat{C}_{\sigma{(j)}}&\leq& \max_{1\leq k\leq j}r_{\sigma(k)}+\frac{1}{\mu}\left((m-1) \right.\nonumber \\
&&\left.\left(p_{\sigma(j),1}^R+\sum_{k=1}^jp_{\sigma(k),1}^M \right) + \sum_{k=1}^j p_{\sigma(k)} \right)
%
%
%\frac{\sum_{k=1}^j p_{\sigma(k)}+(m-1)\sum_{k=1}^j p_{\sigma(k),1}^M}{\mu}+\max_{1\leq k\leq j}r_{\sigma(k)}.
\end{eqnarray}
\end{lemma}
\begin{proof} For now, assume all jobs are released at time zero.  Let $t^*$ be the reduce task of job $\sigma(j)$ that finishes the last. Further, let $D_j^l$ denote the total demand for machine $l$ and idle time involved once all the tasks of $\sigma(1)$ through $\sigma(j)$ except the task $t^*$ are scheduled. Then, we have

%$t^*$ is the last completed task, and $l(t^*)$ is the number of machine used for the task.
%\begin{equation}\notag
%D_j^l\leq\sum_{k=1}^j p_{\sigma(k)l}+p_{\sigma(k),1}\cdot \delta_{l,l(t^*)}
%\end{equation}
%\begin{equation}\notag
%\sum_{l=1}^m D_j^l\leq\sum_{k=1}^j p_{\sigma(k)}+(m-1)\sum_{k=1}^j p_{\sigma(k),1}^M
%\end{equation}

\begin{equation}
\sum_{l=1}^m D_j^l\leq\sum_{k=1}^j p_{\sigma(k)} - p_{\sigma(j),t^*}^R+(m-1)\sum_{k=1}^j p_{\sigma(k),1}^M. 
\end{equation}
This is because $\sum_{k=1}^j p_{\sigma(k)} - p_{\sigma(j),t^*}^R$ is the overall load of the jobs. However, there is an additional idle time between the map jobs and the reduce jobs for all the jobs $\sigma(k)$ for $k\le j$ that need to be accounted in the overall load. The idle time after  map job $\sigma(k)$ is less than the time for processing job of  data size $p_{\sigma(k),1}^M$ at the server. If not, there is a server that is idle for time that is larger than that required to process $p_{\sigma(k),1}^M$ after all map tasks of job $\sigma(k)$ are completed. Then, the last completed map task of $\sigma(k)$ could be shifted to this server decreasing the overall map completion time thus invalidating the policy where the machine is assigned such that it results in the task being completed as early as possible. Further, the machine that finishes the map task the latest would not have idle time, and thus the total idle time at $(m-1)$ machines is each at most  that to process $p_{\sigma(k),1}^M$ making this extra load summed over all the machines as at most $(m-1)\sum_{k=1}^j p_{\sigma(k),1}^M$. 

The completion time of the job $\sigma(j)$ depends on the last completed reduce task $t^*$, and thus, we have $\widehat{C}_{\sigma(j)}v_l \le D_j^l + p_{\sigma(j),t^*}^R$ (The job $t^*$ assigned on any server will give an upper bound on the completion time of the job). Summing this equation over all $l$, we get
\vspace{-.1in}
\begin{equation}
\widehat{C}_{\sigma(j)}\mu \leq  \sum_{k=1}^j p_{\sigma(k)} +(m-1)\sum_{k=1}^j p_{\sigma(k),1}^M + (m-1) p_{\sigma(j),t^*}^R .
\end{equation}


Now suppose that some $r_{j} > 0$. We take our policy to the extreme and suppose that all machines are left idle until every one of jobs $\sigma(1)$ through $\sigma(j)$ are released. Note that
this occurs precisely at time $\max_{1\leq k\leq j}r_{\sigma(k)}$. It is clear that beyond this point in time, we
are effectively in the case where all jobs are released at time zero, hence we can bound the remaining time to completion by the above expression and thus we have 
\vspace{-.2in}
\begin{eqnarray}
&&\widehat{C}_{\sigma(j)}\mu \leq \max_{1\leq k\leq j}r_{\sigma(k)}+ \sum_{k=1}^j p_{\sigma(k)} \nonumber\\
&&+(m-1)\sum_{k=1}^j p_{\sigma(k),1}^M + (m-1) p_{\sigma(j),t^*}^R \label{inlemma}.
\end{eqnarray}


Since, $p_{\sigma(j),t^*}^R \le p_{\sigma(j),1}^R$, we get the result as in the statement of the Lemma. 
\end{proof}

%\textbf{Algorithm CC-LP}: Use the optimal solution $\{C_j^*\}$ of the Map-Reduce Problem to define $m$ permutations $\{\sigma_i:i\in M\}$ which sort jobs in increasing order of $C_j^*-p_{j}/2\mu_j$. For each cluster, execute \textbf{List-LPT($\sigma$)}.


Let $D$ be the largest number s.t. $p_{a,1}^M+p_{a,1}^R\le p_a/D$ for all jobs $a$.  
%Suppose that there exists a $D\ge 1$ such that $p_{a,1}^M+p_{a,1}^R\le p_a/D$. 
We note that the above trivially holds for $D=1$, and thus $D\ge 1$. We now use the above Lemma to give an approximation analysis for the proposed DMRS algorithm. Larger possible value of $D$ helps achieve a tighter bound.  We call $D$ as a task-skewness product, since it can be viewed as the number of tasks times the mean task-size divided by the sum of task-sizes for the largest map and the largest reduce tasks. Thus, for the same skewness, larger number of tasks increase $D$, and more larger jobs increase mean with the same maximum thus helping the skewness and thus the value of $D$. Let $\{C_j\}$ be the completion times given by the LP-MapReduce solution, and $\{C_j^*\}$ be the completion times of the optimal solution. Let $\Gamma_{\rm OPT}$ be the objective value $\sum w_j C_j^*$ for the optimal schedule. Since any feasible solution satisfies the constraints of LP-MapReduce, we have $\sum w_j C_j \le \sum w_j C_j^* = \Gamma_{\rm OPT}$.  Then, we have the following approximation result. 


\begin{theorem}
If $r_{\sigma(k)}\equiv0$, then $\sum_{j\in\mathcal{N}}w_j\hat{C}_j\leq2[1+(m-1)/D]\cdot \Gamma_{\rm OPT}$. Otherwise $\sum_{j\in\mathcal{N}}w_j\hat{C}_j\leq[3+2(m-1)/D]\cdot \Gamma_{\rm OPT}$. \label{thm:approx}
\end{theorem}
\begin{proof} Since $\sum w_j C_j \le \Gamma_{\rm OPT}$, it is enough to show that $\sum_{j\in\mathcal{N}}w_j\hat{C}_j\leq2[1+(m-1)/D]\sum w_j C_j$. 

%We note that the linear program is a relaxation which do not have all the constraints and thus gives a lower bound to the objective function. Thus, we compare the completion times $\widehat{C}_j$ to the solution of linear program $C_j$ thus showing the result.

From \eqref{const1}, we have 
\begin{equation}
\sum_{j\in {\mathcal{S}}}p_{j} C_j \geq \frac{\left(\sum_{j\in {\mathcal{S}}}p_j\right)^2}{2\mu}+\sum_{j\in {\mathcal{S}}}\frac{\left(p_j\right)^2}{2\mu_j}
\end{equation}

Taking $\mathcal{S} = \{\sigma(1), \cdots, \sigma(j)\}$, we have 
\begin{eqnarray}
&& \frac{(\sum_{k=1}^{j}p_{\sigma(k)})^2}{2\mu}\nonumber\\
 &\le& \sum_{k=1}^{j}p_{\sigma(k)} \left(C_{\sigma(k)} - \frac{p_{\sigma(k)}}{2\mu_{\sigma(k)}}\right)\\
 & \le & \left(C_{\sigma(j)} - \frac{p_{\sigma(j)}}{2\mu_{\sigma(j)}}\right) \sum_{k=1}^{j}p_{\sigma(k)}
\end{eqnarray}

This further reduces to
\begin{equation}
\frac{\sum_{k=1}^{j}p_{\sigma(k)}}{\mu}\le 2C_{\sigma(j)} - \frac{p_{\sigma(j)}}{\mu_{\sigma(j)}} \label{psi}
\end{equation}

We first consider the case when $r_{\sigma(k)}\equiv0$. Using Lemma \ref{lemused}, we have 

\begin{eqnarray}
&&\widehat{C}_{\sigma(j)}\mu \nonumber\\
&\leq& \sum_{k=1}^j p_{\sigma(k)} +(m-1)\sum_{k=1}^j p_{\sigma(k),1}^M + (m-1) p_{\sigma(j),1}^R\nonumber\\
&\leq& \sum_{k=1}^j p_{\sigma(k)} +\frac{m-1}{D}\sum_{k=1}^j p_{\sigma(k)} \nonumber\\
&=& \left(1+\frac{m-1}{D}\right)\sum_{k=1}^j p_{\sigma(k)}  \label{simpl}
\end{eqnarray}
Substituting the bound on $\sum_{k=1}^{j}p_{\sigma(k)}$ in \eqref{psi} into \eqref{simpl}, we have 
\vspace{-.1in}
\begin{eqnarray}
\widehat{C}_{\sigma(j)} &\leq&  \left(1+\frac{m-1}{D}\right) \left(2C_{\sigma(j)} - \frac{p_{\sigma(j)}}{\mu_{\sigma(j)}}\right)\nonumber\\
&\leq &  2C_{\sigma(j)}\left(1+\frac{m-1}{D}\right).
\end{eqnarray}

This proves the result for $r_{\sigma(k)}\equiv0$ for all $k$. If that is not the case, we note from \eqref{const4} and \eqref{const5} that
$C_j \geq p_{j}/\mu_j+r_j $. Thus, $r_j \le C_j - p_{j}/\mu_j\le C_j - \frac{p_{j}}{2\mu_j}$. 

Thus, we have for every $k\le j$, 
\begin{eqnarray}
r_{\sigma(k)}&\le & C_{\sigma(k)} - \frac{p_{\sigma(k)}}{2\mu_{\sigma(k)}}\nonumber\\
&\le & C_{\sigma(j)} - \frac{p_{\sigma(j)}}{2\mu_{\sigma(j)}}\nonumber\\
&\le & C_{\sigma(j)}
\end{eqnarray}
Thus, we get the approximation with additional gap of $ C_{\sigma(j)}$ thus giving the result as in the statement of the Theorem. 
\end{proof}

%Suppose $\sigma(j)=x$.
%From (17), $\sum_{k=1}^j p_{\sigma(k)}/\mu\leq 2C_x$.
%
%\begin{eqnarray}
%C_{\sigma{(j)}}\leq\frac{\sum_{k=1}^j p_{\sigma(k)}+(m-1)\sum_{k=1}^j p_{\sigma(k),1}^M}{\mu}+\max_{1\leq k\leq j}r_{\sigma(k)}\\
%\leq\frac{\sum_{k=1}^j p_{\sigma(k)}[1+(m-1)/D]}{\mu}+\max_{1\leq k\leq j}r_{\sigma(k)}\leq2C_x[1+(m-1)/D]+\max_{1\leq k\leq j}r_{\sigma(k)}.\\
%\end{eqnarray}
%With \textbf{algorithm CC-LP}, $\max_{1\leq k\leq j}r_{\sigma(k)}\leq C_x$, which complete the proof.


Theorem \ref{thm:approx} shows that the proposed DMRS algorithm achieves an objective value with a competitive ratio $3+2(m-1)/D$. We note that $D$ is a metric quantifying the task-skewness product of map and reduce tasks, defined as the sum processing data sizes of all map and reduce tasks divided by that of the largest map and reduce tasks. Since $D\ge 1$, the competitive ratio is at most $2m+1$, while tighter bounds are obtained for larger $D$, \ie  as the number of tasks per job increases and there is a higher percentage of large-size jobs (\ie left-skewed). For $D>O(m)$, the approximation ratio is at most a constant, and the competitive ratio results are more promising in this regime. 






==> covsumbound.tex <==
%\section{Proof of Lemma \ref{var}}

We have 
\begin{equation}
\mathbb{E}[T_1+T_2+\cdots+T_k]=\sum_{i=1}^k\mathbb{E}[T_i], \label{eq:summean}
\end{equation}
and
\begin{equation}
{\rm Var}(T_1+T_2+\cdots+T_k)=\sum_{i=1}^k{\rm Var}(T_i), \label{eq:sumvar}
\end{equation}
since $T_1,T_2,\cdots,T_k$ are independent.

Since the coefficient of variation of a random variable $T$ is $\sqrt{{\rm Var}(T)}/\mathbb{E}[T]$, we have
\begin{eqnarray}
\frac{\sqrt{{\rm Var}(T_1+T_2+\cdots+T_k)}}{\mathbb{E}[T_1+T_2+\cdots+T_k]}
&\stackrel{(a)}{=}&\frac{\sqrt{{\rm Var}(T_1)+\cdots+{\rm Var}(T_k)}}{\mathbb{E}[T_1]+\cdots+\mathbb{E}[T_k]}\\
&\stackrel{(b)}{\le}& \max_{i\in\{1\cdots,k\}}\frac{\sqrt{{\rm {\rm Var}}(T_i)}}{\mathbb{E}[T_i]}\\
&\leq& \Delta,
\end{eqnarray}
where (a) follows from \eqref{eq:summean} and \eqref{eq:sumvar}, and (b) is shown in the following.  Suppose $\max_{i\in\{1\cdots,k\}}\\{\sqrt{{\rm Var}(T_i)}}/{\mathbb{E}[T_i]}=\alpha$. Then, we have
\begin{eqnarray}
\frac{\sqrt{{\rm Var}(T_1)+\cdots+{\rm Var}(T_k)}}{\mathbb{E}[T_1]+\cdots+\mathbb{E}[T_k]}
\leq &\frac{\sqrt{\alpha^2 (\mathbb{E}[T_1])^2+\cdots+\alpha^2 (\mathbb{E}[T_k])^2}}{\mathbb{E}[T_1]+\cdots+\mathbb{E}[T_k]}\\
\leq &\alpha \frac{\sqrt{(\mathbb{E}[T_1])^2+\cdots+(\mathbb{E}[T_k])^2}}{\mathbb{E}[T_1]+\cdots+\mathbb{E}[T_k]}\\
\leq &\alpha\\
=& \max_{i\in\{1\cdots,k\}}{\sqrt{{\rm Var}(T_i)}}/{\mathbb{E}[T_i]}.
\end{eqnarray} 

